Deciphering Solar Magnetic Activity: On Grand Minima in Solar Activity

The Sun provides the energy necessary to sustain our existence. While the Sun provides for us, it is also capable of taking away. The weather and climatic scales of solar evolution and the Sun-Earth connection are not well understood. There has been tremendous progress in the century since the discovery of solar magnetism - magnetism that ultimately drives the electromagnetic, particulate and eruptive forcing of our planetary system. There is contemporary evidence of a decrease in solar magnetism, perhaps even indicators of a significant downward trend, over recent decades. Are we entering a minimum in solar activity that is deeper and longer than a typical solar minimum, a "grand minimum"? How could we tell if we are? What is a grand minimum and how does the Sun recover? These are very pertinent questions for modern civilization. In this paper we present a hypothetical demonstration of entry and exit from grand minimum conditions based on a recent analysis of solar features over the past 20 years and their possible connection to the origins of the 11(-ish) year solar activity cycle.

==> Cycletable.tex <==
\begin{table}[!t]
\textbf{\refstepcounter{table}\label{Tab:02} Table \arabic{table}.}{This table contains the times of consecutive (same-signed) maxima, their difference ($\delta$; years) and high-low latitude transit time ($\tau$; years) for each hemisphere.}
\processtable{}
{%\begin{tabular}{cccccc}\toprule
%Cycle & Quantity & Maxima [North] & Maxima [South] & $\Delta$T$_{N}$ & $\Delta$T$_{S}$ \\\midrule
%12 & Sunspot Area & 1884.00 & 1883.83 & \-- & \-- \\
%13 & Sunspot Area & 1892.50 & 1893.58 & \-- & \-- \\
%14 & Sunspot Area & 1905.75 & 1907.08 & \-- & \-- \\
%15 & Sunspot Area & 1917.58 & 1919.50 & \-- & \-- \\
%16 & Sunspot Area & 1925.92 & 1926.08 & \-- & \-- \\
%17 & Sunspot Area & 1937.50 & 1939.67 & \-- & \-- \\
%18 & Sunspot Number & 1949.50 & 1947.50 & \-- & \-- \\
%18 & Sunspot Area & 1949.17 & 1947.17 & \-- & \-- \\
%19 & Sunspot Number & 1959.50 & 1957.50 & \-- & \-- \\
%19 & Sunspot Area & 1959.08 & 1956.83 & \-- \\
%20 & Sunspot Number & 1968.75 & 1970.00 & \-- & \-- \\
%20 & Sunspot Area & 1968.00 & 1970.08 & \-- \\
%21 & Sunspot Number & 1979.50 & 1980.50 & \-- & \-- \\
%21 & Sunspot Area & 1979.67 & 1980.33 & \-- & \-- \\
%22 & Sunspot Number & 1989.50 & 1991.50 & \-- & \-- \\
%22 & Sunspot Area & 1989.08 & 1991.08 & \-- & \-- \\
%23 & Sunspot Number & 2000.75 & 2002.00 & \-- & \-- \\
%23 & Sunspot Area & 2000.50 & 2002.58 & \-- & \-- \\
%24 & Sunspot Number & 2011.75 & 2014.00 & \-- & \-- \\ 
%4 & Sunspot Area & 2000.50 & 2002.58 & \-- & \-- \\ \botrule
    \begin{tabular}{ccccccc}\toprule
    Cycle Pair & Maxima (N) & Maxima (S)  & $\delta_{N}$ & $\delta_{S}$ & $\tau_{N}$ & $\tau_{S}$  \\ \midrule
    14 -- 12  & 1905.75, 1884.00 & 1907.08, 1883.83 & 21.75 & 23.25 &  19.25 & 17.92 \\
    15 -- 13  & 1917.58, 1892.50 & 1919.50, 1893.58 & 25.08 & 25.92 &  19.92 & 18.00 \\
    16 -- 14  & 1925.92, 1905.75 & 1926.08, 1907.08 & 20.17 & 19.00 &  19.18 & 19.02 \\
    17 -- 15  & 1937.50, 1917.58 & 1939.67, 1919.50 & 19.92 & 20.17 &  20.50 & 18.33 \\
    18 -- 16  & 1949.17, 1925.92 & 1947.17, 1926.08 & 23.25 & 21.08 &  19.03 & 21.03 \\
    19 -- 17  & 1959.08, 1937.50 & 1956.83, 1939.67 & 21.58 & 17.17 &  19.42 & 21.67 \\
    20 -- 18  & 1968.00, 1949.17 & 1970.08, 1947.17 & 18.83 & 22.92 &  19.50 & 17.42 \\
    21 -- 19  & 1979.67, 1959.08 & 1980.33, 1956.83 & 20.58 & 23.50 &  19.33 & 18.67 \\
    22 -- 20  & 1989.08, 1968.00 & 1991.08, 1970.08 & 21.08 & 21.00 &  21.92 & 19.92 \\
    23 -- 21  & 2000.50, 1979.67 & 2002.58, 1980.33 & 20.83 & 22.25 &  -- & -- \\ 
    24 -- 22  & 2011.50, 1989.08 & 2014.25, 1991.08 & 22.42 & 23.17 &  -- & -- \\ \botrule
\end{tabular}}{}
\end{table}
